Single-Agent On-line Path Planning in Continuous, Unpredictable and Highly Dynamic Environments

This document is a thesis on the subject of single-agent on-line path planning in continuous,unpredictable and highly dynamic environments. The problem is finding and traversing a collision-free path for a holonomic robot, without kinodynamic restrictions, moving in an environment with several unpredictably moving obstacles or adversaries. The availability of perfect information of the environment at all times is assumed. Several static and dynamic variants of the Rapidly Exploring Random Trees (RRT) algorithm are explored, as well as an evolutionary algorithm for planning in dynamic environments called the Evolutionary Planner/Navigator. A combination of both kinds of algorithms is proposed to overcome shortcomings in both, and then a combination of a RRT variant for initial planning and informed local search for navigation, plus a simple greedy heuristic for optimization. We show that this combination of simple techniques provides better responses to highly dynamic environments than the RRT extensions.

==> tex/Abstract.tex <==
% Thesis Abstract ------------------------------------------------------

\prefacesection{Abstract}
This document is a thesis on the subject of single-agent
on-line path planning in continuous,unpredictable and highly dynamic
environments. The problem is finding and traversing a collision-free path
for a holonomic robot,
without kinodynamic restrictions, moving in an environment with several
unpredictably moving obstacles or adversaries.
The availability of perfect information of the environment at all times is
assumed.

Several static and dynamic variants of the Rapidly Exploring Random Trees (RRT)
algorithm are explored, as well as an evolutionary algorithm for planning in
dynamic environments called the Evolutionary Planner/Navigator. A combination of
both kinds of algorithms is proposed to overcome shortcomings in both, and then
a combination of a RRT variant for initial planning and informed local search for
navigation, plus a simple greedy heuristic for optimization.
We show that this combination of simple techniques provides
better responses to highly dynamic environments than the RRT extensions.
%Also
%proposed is the construction of a path planning testing framework, and its use
%for comparing previously uncompared algorithms.

\textbf{Keywords:} Artificial intelligence, motion planning, RRT, Multi-stage,
informed local search, greedy heuristics, evolutionary algorithms

% ----------------------------------------------------------------------


==> tex/Acknowledgements.tex <==
% Thesis Acknowledgements ----------------------------------------------

\prefacesection{Acknowledgments}
\def\baselinestretch{1.0}
\setlinespacing{1.15}

\noindent
A mis hermanos, por quienes he tratado de ser una mejor persona, para ser un
buen ejemplo para ellos. A mis padres, de quienes hered\'e lo que soy, tanto en cuerpo como en
esp\'\i ritu. A mis abuelos y abuelas, especialmente mi Opapa, de quien
aprend\'{\i} a disfrutar la
vida, y mi Tata, quien me ense\~n\'o el valor de la familia.\\
\bigskip\medskip

\noindent
Quiero tambi\'en agradecer a los que hicieron posible esta tesis: Mauricio Araya
por ayudarme a escoger el tema y en el desarrollo posterior, a Rodrigo Araya por
obligarme a trabajar en medio de las vacaciones de verano, a
Nicol\'as Troncoso, Diego Candel
y Roberto Bonvallet, y a mis profesores
gu\'\i as y correferentes, Mauricio Solar, Horst H. von Brand y John Atkinson por sus 
aportes durante el desarrollo de esta tesis.\\

\noindent
Quiero aprovechar la oportunidad para agradecer a los profesores que marcaron mi 
estad\'\i a en la Universidad: Horst H. von Brand, H\'ector Allende, Luis Salinas, Hubert
Hoffmann, Claudio Dib y Viktor Sl\"usarenko.\\
\medskip

\noindent
Finalmente, quiero agradecer en especial a Pamela Saavedra, por estar junto a
m\'{\i}
durante los m\'as de diez meses que demor\'o en ser terminada esta tesis, soport\'andome y
apoy\'andome en los momentos m\'as dif\'\i ciles.
\bigskip\medskip

\noindent
Valpara\'{\i}so, Chile \hfill Nicol\'as A. Barriga\\
Noviembre 2009

% ----------------------------------------------------------------------


==> tex/Resumen.tex <==
\prefacesection{Resumen}
Este documento es una tesis en el tema de planificaci\'on de caminos uniagente y en
l\'inea, para ambientes continuos, impredecibles y altamente din\'amicos. El problema es encontrar
y recorrer un camino sin colisiones para un robot holon\'omico, sin restricciones kinodin\'amicas,
movi\'endose en un ambiente con varios obst\'aculos o adversarios movi\'endose
impredeciblemente. Se asume la disponibilidad de informaci\'on perfecta del entorno en todo
momento.

Varias variantes est\'aticas y din\'amicas del algoritmo ``Rapidly Exploring Random
Trees'' (RRT)
se exploran, as\'i como tambi\'en un algoritmo evolutivo para planificaci\'on en ambientes
din\'amicos llamado ``Evolutionary Planner/Navigator.'' Se propone una combinaci\'on de ambos
algoritmos para superar las falencias de ambos y luego una combinaci\'on de RRT
para planificaci\'on inicial y b\'usqueda local informada para navegaci\'on, sumado a una 
heur\'istica voraz simple para optimizaci\'on. Se demuestra que esta combinaci\'on de t\'ecnicas 
simples produce mejores respuestas en ambientes altamente din\'amicos que las variantes RRT
est\'andar.
%Adem\'as se propone la construcci\'on de
%un framework, y su utilizaci\'on para comparar algoritmos que previamente no hab\'ian sido
%comparados.

\textbf{Palabras Claves:} Inteligencia artificial. planificaci\'on de rutas,
RRT, multi-etapa, b\'usqueda local informada, heur\'istica voraz, algoritmos
evolutivos

